How to Calibrate Your Event Camera

We propose a generic event camera calibration framework using image reconstruction. Instead of relying on blinking LED patterns or external screens, we show that neural-network-based image reconstruction is well suited for the task of intrinsic and extrinsic calibration of event cameras. The advantage of our proposed approach is that we can use standard calibration patterns that do not rely on active illumination. Furthermore, our approach enables the possibility to perform extrinsic calibration between frame-based and event-based sensors without additional complexity. Both simulation and real-world experiments indicate that calibration through image reconstruction is accurate under common distortion models and a wide variety of distortion parameters

==> floats/fig_frames_davis_gen3.tex <==
\global\long\def\figWidth{0.24\linewidth}
\begin{figure}[t]
	\centering
\resizebox{1.1\columnwidth}{!}{
    \setlength{\tabcolsep}{2pt}
	\begin{tabular}{
	M{\figWidth}
	M{\figWidth}}
%		\midrule
		& Davis346 frame & Prophesee Gen3 EM frame
		\\%\addlinespace[1ex]
		&\frame{\includegraphics[width=\linewidth]{images/davis_frame.png}}
		&\frame{\includegraphics[width=\linewidth]{images/prophesee_em_frame.png}}
		\\%\addlinespace[1ex]
	\end{tabular}
	\vspace{-1ex}
} % resizebox
	\caption{
	}
	\label{fig:experim:simulation:e2vid}
	%\vspace{-1ex}
\end{figure}

==> floats/fig_kalibr_simulation.tex <==
\global\long\def\figWidth{0.24\linewidth}
\begin{figure}[t]
	\centering
\resizebox{1.1\columnwidth}{!}{
    \setlength{\tabcolsep}{2pt}
	\begin{tabular}{
	M{0.35cm}
	M{\figWidth}
	M{\figWidth}
	M{\figWidth}}
%		\midrule
		& No Distortion & Equidistant distortion & Radial-tangential distortion
		\\%\addlinespace[1ex]
		\rotatebox{90}{\makecell{Checkerboard}}
		&\includegraphics[width=\linewidth]{images/kalibr_check_no_distortion.png}
		&\includegraphics[width=\linewidth]{images/kalibr_check_equi.png}
		&\includegraphics[width=\linewidth]{images/kalibr_check_radtan.png}
		\\%\addlinespace[1ex]
		\rotatebox{90}{\makecell{AprilTag}}
		&\includegraphics[width=\linewidth]{images/kalibr_april_no_distorion.png}
		&\includegraphics[width=\linewidth]{images/kalibr_april_equi.png}
		&\includegraphics[width=\linewidth]{images/kalibr_april_radtan.png}
		\\%\addlinespace[1ex]
	\end{tabular}
	\vspace{-1ex}
} % resizebox
	\caption{ToDo reference in the text}
	\label{fig:experim:simulation:kalibr}
	%\vspace{-1ex}
\end{figure}

==> floats/table_focal_lengths.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \setlength{\tabcolsep}{3pt}
    {\small
    \begin{tabular}{llrrrr}
        \toprule
        Sensor  &  Modality & \multicolumn{1}{c}{Davis346}  & \multicolumn{1}{c}{Samsung Gen3}& \multicolumn{1}{c}{Prophesee Gen3} & \multicolumn{1}{c}{Prophesee Gen4}   \\
        \midrule
                   Blinking LED          & \emph{E}  &  &  &   &  \\
                   LCD screen          & \emph{E}  &  &  &   &  \\
                   Checkerboard(E2VID)  & \emph{E} &  &  &   &  \\\midrule
                   Checkerboard(Frames) & \emph{I} &  &  &   &  \\
        \bottomrule
    \end{tabular}
    }
    \end{adjustbox}
    \vspace{-1ex}
    \caption{Focal length. The input modalities \emph{E} and \emph{I} represent events and images respectively that are used for the calibration method.}
    \label{tab:comparison:focal_length}
    \vspace{-2ex}
\end{table*}

